Contrastive learning for regression in multi-site brain age prediction

Building accurate Deep Learning (DL) models for brain age prediction is a very relevant topic in neuroimaging, as it could help better understand neurodegenerative disorders and find new biomarkers. To estimate accurate and generalizable models, large datasets have been collected, which are often multi-site and multi-scanner. This large heterogeneity negatively affects the generalization performance of DL models since they are prone to overfit site-related noise. Recently, contrastive learning approaches have been shown to be more robust against noise in data or labels. For this reason, we propose a novel contrastive learning regression loss for robust brain age prediction using MRI scans. Our method achieves state-of-the-art performance on the OpenBHB challenge, yielding the best generalization capability and robustness to site-related noise.

==> 2_related.tex <==
\section{Related works}
\label{sec:related}

%
Our contribution is based on the related literature in contrastive learning, metric learning, fairness, and debiasing. 
Contrastive methods learn a representation space of input data by attracting semantically similar \textit{positive} samples (e.g. with the same labels~\cite{khosla2020supervised}) and by repelling dissimilar \textit{negative} samples (e.g. with distinct labels). When label information is not available, instance-based discrimination approaches~\cite{chen2020simCLR, chen2020mocov2, zbontar_barlow_2021, dwibedi2021little, caron2020unsupervised, grill2020bootstrap} have gained considerable success, almost closing the gap with its supervised counterpart. Most recent research in CL has focused on designing the right data augmentations~\cite{chen2020simCLR,zhang2022rethinking}, contrastive losses~\cite{chen2020simCLR, grill2020bootstrap, zbontar_barlow_2021}, memory banks~\cite{chen2020mocov2, grill2020bootstrap, dwibedi2021little}, prototypes (or clusters)~\cite{caron2020unsupervised, li2020prototypical} typically for downstream  classification, detection or segmentation tasks-- leaving open the question for regression tasks. When weak labels are available (either discrete or continuous), kernel approaches have been explored for CL~\cite{dufumier2021contrastive, dufumier2022rethinking}, using a re-weighting scheme to adapt alignment term between samples with close weak labels. 


==> derivations.tex <==
\section{Derivations}

We make the hypothesis that we only have weakly  attributes $y$. If they are discrete, we could say that one sample $x_k$ would be considered positive only if it has exactly the same attribute of the anchor (i.e., $y=y_k$). Otherwise it is considered as a negative. In that case, we would obtain exactly SupCon:

\begin{equation}
        s_t - s_k \leq 0 \quad  \text{ if } w_k=\delta(y-y_k)=1 \quad \forall k,t \neq k        
\end{equation}

If we define as negatives the samples that have a different attribute than the one of the anchor and positives the ones that have the same attribute, we retrieve: 

\begin{equation}
    s^-_j - s^+_i \leq 0 \quad \forall i,j \quad \text{ and } \quad s^+_t - s^+_i \leq 0 \quad \forall i,t \neq i
    \label{eq:supcon-condition-full}
\end{equation}

Exactly as in the ICLR paper.
This can be translated as an optimization problem using:


\begin{align}
    \argmin_f \sum_k w_k \max(0, \{ s_t - s_k \}_{\substack{t=1,...,N \\ t \neq k}})\\ \approx \argmin_f \left[ \sum_k w_k \log \left( \exp(0) + \sum_{t \neq k} \exp(s_t - s_k)\right) \right]    
\end{align}

\begin{equation}
\setlength{\jot}{15pt}
\begin{aligned}
  &\approx \sum_k w_k \log \left( \exp(0) + \sum_{t \neq k} \exp(s_t - s_k) \right) \\
    & = \sum_k w_k \log \left( 1 + \frac{\sum_{t \neq k} \exp(s_t)}{\exp(s_k)} \right) \\
    & = \sum_k w_k \log \left( \frac{ \exp(s_k) + \sum_{t \neq k} \exp(s_t)}{\exp(s_k)}  \right) \\
    &= - \sum_k w_k \log \left( \frac{\exp(s_k)}{\exp(s_k) + \sum_{t \neq k} \exp(s_t)}  \right) \\
    &= - \sum_k w_k \log \left( \frac{\exp(s_k)}{\sum_{t=1}^N \exp(s_t)}  \right)
\end{aligned}
\end{equation}

In the MICCAI paper we have made the hypothesis that

\begin{equation}
        s_t - s_k \leq 0 \quad  \text{ if } \frac{w_k}{\sum_j w_j} \neq 0 \quad \forall j,k,t \neq k        
\end{equation}

\begin{align}
    \sum_k \frac{w_k}{\sum_t w_t} \max(0, \{ s_t - s_k \}_{\substack{t=1,...,N \\ t \neq k}}) \\ \approx  - \sum_k \frac{w_k}{\sum_t w_t} \log \left( \frac{\exp(s_k)}{\sum_{t=1}^N \exp(s_t)}  \right)
\end{align}

%
\begin{equation}
    - \sum_k \delta_{\frac{w_k}{\sum_t w_t} > 0} \log \left( \frac{\exp(s_k)}{\sum_{t=1}^N \exp(s_t)}  \right)
\end{equation}

\subsection{Analysis of $\mathcal{L}^{thr}$}

But in reality, we would like to optimize:

\begin{equation}
        s_t - s_k \leq 0 \quad  \text{ if } w_t - w_k \leq 0 \text{ and } w_k \neq 0 \quad \forall k,t \neq k        
\end{equation}

%

\begin{equation}
\begin{aligned}
    \mathcal{L}^{thr}_i &= - \sum_k \frac{w_k}{\sum_t \delta_{w_t < w_k} w_t} \log \left( \frac{\exp(s_k)}{\sum_{t=1}^N \delta_{w_t < w_k} \exp(s_t)}  \right) \\
    &= \sum_k \frac{w_k}{?}\left[\log\exp(-s_k) + \log\left(\sum_{t=1}^N \delta_{w_t < w_k} \exp(s_t) \right)\right] \\
    &= \sum_k \frac{w_k}{?}\log\left(\exp(-s_k)\sum_{t=1}^N \delta_{w_t < w_k} \exp(s_t) \right) \\
    &= \sum_k \frac{w_k}{?} \log\left(\sum_{t=1}^N \delta_{w_t < w_k} \exp(s_t - s_k) \right) \\
    &\approx \sum_k \frac{w_k}{?} \max(0, \{s_t - s_k\}_{w_t < w_k})
\end{aligned}
\end{equation}


\noindent  meaning that given an anchor $z_i$ and a sample $z_k$ we want to maximize the margin between $z_k$ and the closest sample $z_j$ which is ``more negative'' than $z_k$. %

%


I don't think that $w$ needs to be an actual kernel so I removed the normalization. 
This means that, during optimization, for each sample $k$ we should first look whether $w_k \neq 0$, so if the attributes of the sample $k$ and the anchor are similar according to the similarity function (or kernel) $w$. Then, we should create the negatives samples $t$ by looking at the samples in the batch that have $w_t - w_k \leq 0$. Other solutions are possible of course !

\subsection{Analysis of $\mathcal{L}^{exp}$}

\begin{equation}
\begin{aligned}
    \mathcal{L}^{exp} &= -\frac{1}{\sum_t w_t}\sum_{k}w_k \log \frac{\exp(s_k)}{\sum_{t \neq k} \exp(s_t(1-w_t))} \\
    &= \frac{1}{\sum_t w_t}\sum_{k}w_k \left[\log\exp(-s_k) + \log\sum_{t \neq k}\exp(s_t(1-w_t))\right] \\
    &= \frac{1}{\sum_t w_t}\sum_{k}w_k \log\left(\exp(-s_k)\sum_{t \neq k}\exp(s_t(1-w_t)) \right) \\
    &= \frac{1}{\sum_t w_t}\sum_{k}w_k \log\left(\sum_{t \neq k}\exp(s_t(1-w_t) - s_k) \right) \\
    &\approx \frac{1}{\sum_t w_t}\sum_{k}w_k \max(0, \{s_t(1-w_t) - s_k\}) \\
    & s_t(1-w_t) - s_k \leq 0  \quad  \text{ if } w_k > 0
\end{aligned}
\end{equation}
%

%


We make the hypothesis there is just one $k$ and one $t$
\begin{equation}
\begin{aligned}
& w_k(s_t - s_k)\leq 0 \quad w_k \geq 0 \\ 
& \argmin_f \max(0, \{ w_k (s_t - s_k) \}=\argmin_f w_k \max(0, \{(s_t - s_k) \}\\ 
& \approx \argmin_f \log \left( \exp(0) +  \exp( w_k (s_t - s_k))\right) = \log \left( \exp(0) +  \exp(s_t - s_k)^{w_k} \right)\neq\\
& \approx \argmin_f w_k \log \left( \exp(0) +  \exp(s_t - s_k)\right)
\end{aligned}
\end{equation}

Without the $\exp(0)$, it would be the same. 

\noindent %
\begin{equation}
\begin{aligned}
    \argmin_f \log \left( \exp(0) + \exp( w_k (s_t - s_k))\right) \\
    = \argmin_f \log \left(\exp(0) + \frac{\exp(w_k s_t)}{\exp(w_k s_k)}\right)\\
    = \argmin_f \log \left(\frac{\exp(w_k s_k) + \exp(w_k s_t)}{\exp(w_k s_k)}\right) \\
    = \argmin_f - \log \left(\frac{\exp(w_k s_k)}{\exp(w_k s_k) + \exp(w_k s_t)} \right) \\
    = \argmin_f - \log \left(\frac{\exp(s_k)^{w_k}}{\exp(s_k)^{w_k} + \exp(s_t)^{w_k}} \right) \\
    = \argmin_f - \left[\log\exp(s_k)^{w_k} - \log(\exp(s_k)^{w_k} + \exp(s_t)^{w_k}) \right] \\
\end{aligned}
\end{equation}


If I add the sum over the t within the log, is even more different

\begin{equation}
\begin{aligned}
& w_k(s_t - s_k)\leq 0 \quad w_k \geq 0 \forall k,t \\ 
& \argmin_f \sum_k \max(0, \{ w_k (s_t - s_k) \})_{t=1,...,N}=\argmin_f \sum_k w_k \max(0, \{(s_t - s_k) \})_{t=1,...,N}\\ 
& \approx \argmin_f \sum_k \log \left( \exp(0) + \sum_t \exp(s_t - s_k)^{w_k}\right) \neq\\
& \approx \argmin_f \sum_k w_k \log \left( \exp(0) + \sum_t \exp(s_t - s_k)\right)
\end{aligned}
\end{equation}

